RAT: Boosting Misclassification Detection Ability without Extra Data

As deep neural networks(DNN) become increasingly prevalent, particularly in high-stakes areas such as autonomous driving and healthcare, the ability to detect incorrect predictions of models and intervene accordingly becomes crucial for safety. In this work, we investigate the detection of misclassified inputs for image classification models from the lens of adversarial perturbation: we propose to use robust radius (a.k.a. input-space margin) as a confidence metric and design two efficient estimation algorithms, RR-BS and RR-Fast, for misclassification detection. Furthermore, we design a training method called Radius Aware Training (RAT) to boost models' ability to identify mistakes. Extensive experiments show our method could achieve up to 29.3% reduction on AURC and 21.62% reduction in FPR@95TPR, compared with previous methods.

==> tables/bb_results.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{c|l|c|c|c}
\hline
\multicolumn{5}{c}{Dataset: CIFAR10}                                            \\ \hline
& Method  & AURC $\times$ 1000 $\downarrow$ & FPR@95\%TPR $\downarrow$ & AUROC $\uparrow$ \\ 
\hline
\multirow{7}{*}{WRN-28} & \multicolumn{4}{l}{\textbf{Baseline}\rule{0pt}{2ex}}                                           \\ \cdashline{2-5}
& MSR & 5.86 $\pm$ 0.40 & 72.89\% $\pm$ 6.48\% & 0.8941 $\pm$ 0.0052 \\
& ODIN & \add{5.16} $\pm$ \add{0.75} & \add{91.04\%} $\pm$ \add{12.74\%} & \add{0.8953} $\pm$ \add{0.0104} \\
& DOCTOR & \add{5.16} $\pm$ \add{0.75} & \add{91.04\%} $\pm$ \add{12.74\%} & \add{0.8953} $\pm$ \add{0.0104} \\
& RelU & 6.65 $\pm$ 2.42 & 73.75\% $\pm$ 15.55\% & 0.8571 $\pm$ 0.0353 \\
\cdashline{2-5}
& \multicolumn{4}{l}{\textbf{Our methods}\rule{0pt}{2ex}}                                            \\ \cdashline{2-5}
& \RobustRadBB \rule{0pt}{2.2ex} & \textbf{4.60 $\pm$ 0.27} & \textbf{66.01\% $\pm$ 3.28\%} &\textbf{0.9032 $\pm$ 0.0058} \\
\hline
% \multirow{5}{*}{DenseNet-40}& MSR & 11.00 $\pm$ 1.26 & 60.57\% $\pm$ 5.16\% & 0.8978 $\pm$ 0.0074 \\
% & ODIN & 11.00 $\pm$ 1.26 & 60.57\% $\pm$ 5.16\% & 0.8978 $\pm$ 0.0074 \\
% & DOCTOR & 11.01 $\pm$ 1.26 & 60.62\% $\pm$ 5.16\% & 0.8978 $\pm$ 0.0075 \\
% & RelU & 9.53 $\pm$ 1.85 & 45.61\% $\pm$ 7.32\% & 0.9002 $\pm$ 0.0100 \\
% \cdashline{2-5}
% & \RobustRadBB \rule{0pt}{2.2ex} & \textbf{8.60 $\pm$ 0.76} & \textbf{43.62\% $\pm$ 2.57\%} & \textbf{0.9115 $\pm$ 0.0058} \\\hline
\multirow{7}{*}{DenseNet-190}& \multicolumn{4}{l}{\textbf{Baseline}\rule{0pt}{2ex}}  \\ \cdashline{2-5}
& MSR & 5.36 $\pm$ 0.36 & 67.37\% $\pm$ 2.22\% & 0.8841 $\pm$ 0.0070 \\
& ODIN & \add{5.04} $\pm$ \add{0.50} & \textbf{\add{62.93\%} $\pm$ \add{0.69\%}} & \add{0.8918} $\pm$ \add{0.0040} \\
& DOCTOR & \add{5.04} $\pm$ \add{0.50} &  \textbf{\add{62.93\%} $\pm$ \add{0.69\%}} & \add{0.8918} $\pm$ \add{0.0040} \\
& RelU & 10.64 $\pm$ 2.53 & 84.24\% $\pm$ 2.75\% & 0.7883 $\pm$ 0.0404 \\
\cdashline{2-5}
& \multicolumn{4}{l}{\textbf{Our methods}\rule{0pt}{2ex}}                                            \\ \cdashline{2-5}
& \RobustRadBB \rule{0pt}{2.2ex} & \textbf{4.85 $\pm$ 0.47} & \textbf{63.72\% $\pm$ 4.04\%} & \textbf{0.9026 $\pm$ 0.0078} \\
\hline
\multicolumn{5}{c}{Dataset: CIFAR100}\\ \hline
\multirow{7}{*}{WRN-28} & \multicolumn{4}{l}{\textbf{Baseline}\rule{0pt}{2ex}}  \\ \cdashline{2-5}
& MSR & 56.46 $\pm$ 0.63 & 63.26\% $\pm$ 2.42\% & 0.8600 $\pm$ 0.001\textbf{}3 \\
& ODIN & \add{47.86} $\pm$ \add{0.39} & \add{51.06\%} $\pm$ \add{1.38\%} & \add{0.8706} $\pm$ \add{0.0020} \\
& DOCTOR & \add{47.80} $\pm$ \add{0.39} &  \add{51.06\%} $\pm$ \add{1.38\%} & \textbf{\add{0.8710} $\pm$ \add{0.0021}} \\
& RelU & 57.79 $\pm$ 4.06 & 61.48\% $\pm$ 7.51\% & 0.8428 $\pm$ 0.0079 \\
\cdashline{2-5}
& \multicolumn{4}{l}{\textbf{Our methods}\rule{0pt}{2ex}}                                            \\ \cdashline{2-5}
& \RobustRadBB \rule{0pt}{2.2ex} & \textbf{46.99 $\pm$ 0.60} & \textbf{48.22\% $\pm$ 0.73\%} & \textbf{0.8693 $\pm$ 0.0012} \\
\hline
% \multirow{5}{*}{DenseNet-40}& MSR & \textbf{70.92 $\pm$ 0.44} & 42.90\% $\pm$ 0.40\% & \textbf{0.8689 $\pm$ 0.0004} \\
% & ODIN & \textbf{70.92 $\pm$ 0.44} & 42.90\% $\pm$ 0.40\% & \textbf{0.8689 $\pm$ 0.0004} \\
% & DOCTOR & 72.04 $\pm$ 0.45 & 42.97\% $\pm$ 0.38\% & 0.8645 $\pm$ 0.0007 \\
% & RelU & 84.82 $\pm$ 1.85 & 49.28\% $\pm$ 1.04\% & 0.8254 $\pm$ 0.0052 \\
% \cdashline{2-5}
% &  \RobustRadBB \rule{0pt}{2.2ex} & 72.64 $\pm$ 0.49 &\textbf{42.64\% $\pm$ 0.62\%} & 0.8605 $\pm$ 0.0005 \\
% \hline
\multirow{7}{*}{DenseNet-190} & \multicolumn{4}{l}{\textbf{Baseline}\rule{0pt}{2ex}}  \\ \cdashline{2-5}
& MSR & 47.04 $\pm$ 0.98 & 53.06\% $\pm$ 1.46\% & 0.8702 $\pm$ 0.0030 \\
& ODIN & \add{43.88} $\pm$ \add{1.12} & \add{43.95\%} $\pm$ \add{1.98\%} & \add{0.8798} $\pm$ \add{0.0014} \\
& DOCTOR & \add{43.84} $\pm$ \add{1.12} & \add{43.95\%} $\pm$ \add{1.98\%} & \add{0.8800} $\pm$ \add{0.0014} \\
& RelU & 50.02 $\pm$ 2.80 & 59.10\% $\pm$ 4.65\% & 0.8555 $\pm$ 0.0062 \\
\cdashline{2-5}
& \multicolumn{4}{l}{\textbf{Our methods}\rule{0pt}{2ex}}                                            \\ \cdashline{2-5}
& \RobustRadBB \rule{0pt}{2.2ex} & \textbf{41.15 $\pm$ 0.83} & \textbf{39.36\% $\pm$ 0.71\%} & \textbf{0.8829 $\pm$ 0.0019} \\
\hline
\end{tabular}
\caption{Misclassification detection results under black box setting. We test our methods on two datasets: CIFAR10 and CIFAR100, with two architectures: WideResNet(WRN)\cite{zagoruyko2016wrn} and DenseNet\cite{huang2017densely}. For each method, we display three metrics: AURC, FPR95 and AUROC. For AURC and FPR95, lower is better. For AUROC, higher is better. Our methods consistently outperform the baselines over these benchmarks. }
\label{tab:BBresults}
\end{table}

==> tables/imagenet.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!h]
\centering
\begin{tabular}{c|l|c|c|c}
\hline
& \multicolumn{4}{l}{Dataset: ImageNet}                                            \\ \hline
& Method               & AURC  $\times$ 1000 $\downarrow$& FPR@95\%TPR $\downarrow$& AUROC $\uparrow$  \\
\hline
\multirow{9}{*}{ViT/B-16} & \multicolumn{4}{l}{\textbf{Baseline}\rule{0pt}{2ex}}  \\ \cdashline{2-5}
& MSR & 56.90  & 54.77\%  & 0.8546  \\
& ODIN & \add{49.90} & \add{45.25\%} & \add{0.8669}  \\
& DOCTOR & \add{50.04}  & \add{45.76\%}  & \add{0.8670}  \\
& RelU & 71.96  & 67.44\%  & 0.7953  \\
\cdashline{2-5}
& \multicolumn{4}{l}{\textbf{Our methods}\rule{0pt}{2ex}}                                            \\ \cdashline{2-5}
& \RobustRad(Ours) & 57.25  & 54.94\%  & 0.8439  \\
&  \RobustRadFast(Ours) & 58.55  & 59.63\%  & 0.8403  \\
&  \RobustRadBB(Ours) & \textbf{50.12}  & \textbf{45.54\%}  &\textbf{0.8624}  \\
\hline
\end{tabular}
\caption{Results for our methods and baselines of ViT-B/16 model on ImageNet.  For each method, we display three metrics: AURC, FPR95 and AUROC. For AURC and FPR95, lower is better. For AUROC, higher is better. Our methods consistently outperform the baselines over these benchmarks.}
\label{tab:ImageNetResults}
\end{table*}

==> tables/main_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!ht]
\centering
\scalebox{0.95}{
\begin{tabular}{c|l|c|c|c}
\hline
& \multicolumn{4}{l}{Dataset: CIFAR10}                                            \\ \hline
 & Method               & AURC  $\times$ 1000 $\downarrow$& FPR@95\%TPR $\downarrow$& AUROC $\uparrow$  \\
\hline
\multirow{9}{*}{WRN-28} & \multicolumn{4}{l}{\textbf{Baseline}\rule{0pt}{2ex}}                                           \\ \cdashline{2-5}
& MSR & 3.69 $\pm$ 0.43 & 51.41\% $\pm$ 8.57\% & 0.9097 $\pm$ 0.0079 \\
& ODIN & \add{3.58} $\pm$ \add{0.39} & \add{58.00\%} $\pm$ \add{24.60\%} & \add{0.9123} $\pm$ \add{0.0062} \\
& DOCTOR & \add{5.59} $\pm$ \add{0.57} & \add{91.07\%} $\pm$ \add{13.12\%} & \add{0.8865} $\pm$ \add{0.0119} \\
& RelU & 9.45 $\pm$ 1.37 & 83.29\% $\pm$ 7.84\% & 0.7846 $\pm$ 0.0256 \\
\cdashline{2-5}
& \multicolumn{4}{l}{\textbf{Our methods}\rule{0pt}{2ex}}                                            \\ \cdashline{2-5}
& \RobustRad\rule{0pt}{2.2ex} & 3.25 $\pm$ 0.40 & \textbf{27.12\% $\pm$ 7.00\%} & \textbf{0.9388 $\pm$ 0.0044} \\
& \RobustRadFast & \textbf{2.93 $\pm$ 0.42} & 41.31\% $\pm$ 9.43\% & 0.9346 $\pm$ 0.0071 \\
& \RobustRadBB & 3.77 $\pm$ 0.71 & 55.43\% $\pm$ 9.26\% & 0.9106 $\pm$ 0.0098 \\
\hline
% \multirow{7}{*}{DenseNet-40}& MSR & 9.33 $\pm$ 0.24 & 42.57\% $\pm$ 2.69\% & 0.9059 $\pm$ 0.0022 \\
% & ODIN & 9.83 $\pm$ 0.94 & 48.03\% $\pm$ 8.94\% & 0.9045 $\pm$ 0.0077 \\
% & DOCTOR & 11.47 $\pm$ 0.18 & 63.55\% $\pm$ 0.25\% & 0.8938 $\pm$ 0.0027 \\
% & RelU & 9.87 $\pm$ 1.58 & 50.31\% $\pm$ 7.37\% & 0.8945 $\pm$ 0.0161 \\
% \cdashline{2-5}
% & \RobustRad \rule{0pt}{2.2ex}  & \textbf{6.13 $\pm$ 0.24} & \textbf{20.60\% $\pm$ 0.72\%} & \textbf{0.9322 $\pm$ 0.0016} \\
% & \RobustRadFast  & 6.90 $\pm$ 0.27 & 24.48\% $\pm$ 0.71\% & 0.9257 $\pm$ 0.0026 \\
% & \RobustRadBB  & 8.56 $\pm$ 0.37 & 41.37\% $\pm$ 6.18\% & 0.9082 $\pm$ 0.0033 \\
% \hline
\multirow{9}{*}{ResNet110}& \multicolumn{4}{l}{\textbf{Baseline}\rule{0pt}{2ex}}           \\ \cdashline{2-5}
& MSR & 4.15 $\pm$ 0.32 & 52.93\% $\pm$ 3.89\% & 0.9083 $\pm$ 0.0063 \\
& ODIN & \add{4.13} $\pm$ \add{0.32} & \add{56.94\%} $\pm$ \add{2.87\%} & \add{0.9109} $\pm$ \add{0.0053} \\
& DOCTOR & \add{5.50} $\pm$ \add{0.33} & \add{79.01\%} $\pm$ \add{19.19\%} & \add{0.8867} $\pm$ \add{0.0052} \\
& RelU & 12.42 $\pm$ 1.67 & 87.42\% $\pm$ 3.61\% & 0.7429 $\pm$ 0.0263 \\
\cdashline{2-5}
& \multicolumn{4}{l}{\textbf{Our methods}\rule{0pt}{2ex}}                                            \\ \cdashline{2-5}
& \RobustRad \rule{0pt}{2.2ex} & \textbf{3.29 $\pm$ 0.62} & \textbf{35.01\% $\pm$ 8.89\%} &\textbf{ 0.9332 $\pm$ 0.0081} \\
& \RobustRadFast  & \textbf{3.29 $\pm$ 0.51} & 50.30\% $\pm$ 4.80\% & 0.9277 $\pm$ 0.0086 \\
& \RobustRadBB  & 4.18 $\pm$ 0.44 & 58.86\% $\pm$ 5.12\% & 0.9085 $\pm$ 0.0083 \\
\hline
& \multicolumn{4}{l}{Dataset: CIFAR100}\\ \hline
\multirow{9}{*}{WRN-28} & \multicolumn{4}{l}{\textbf{Baseline}\rule{0pt}{2ex}}           \\ \cdashline{2-5}
& MSR & 50.93 $\pm$ 1.29 & 51.08\% $\pm$ 0.21\% & 0.8646 $\pm$ 0.0016 \\
& ODIN & \add{47.14} $\pm$ \add{1.19} & \add{47.26\%} $\pm$ \add{2.59\%} & \add{0.8725} $\pm$ \add{0.0022} \\
& DOCTOR & \add{49.03} $\pm$ \add{1.08} & \add{50.90\%} $\pm$ \add{2.24\%} & \add{0.8704} $\pm$ \add{0.0023} \\
& RelU & 59.99 $\pm$ 7.41 & 64.48\% $\pm$ 8.68\% & 0.8348 $\pm$ 0.0178 \\
\cdashline{2-5}
& \multicolumn{4}{l}{\textbf{Our methods}\rule{0pt}{2ex}}                                            \\ \cdashline{2-5}
& \RobustRad \rule{0pt}{2.2ex} & \textbf{42.28 $\pm$ 1.86} & \textbf{36.38\% $\pm$ 1.20\%} & \textbf{0.8834 $\pm$ 0.0023} \\
& \RobustRadFast  & 42.38 $\pm$ 2.65 & 50.11\% $\pm$ 27.91\% & \textbf{0.8834 $\pm$ 0.0039} \\
& \RobustRadBB  & 46.88 $\pm$ 1.05 & 48.16\% $\pm$ 0.67\% & 0.8698 $\pm$ 0.0023 \\
\hline
% \multirow{7}{*}{DenseNet-40}& MSR & \textbf{70.53 $\pm$ 0.56} & \textbf{42.94\% $\pm$ 0.47\%} & \textbf{0.8679 $\pm$ 0.0016 }\\
% & ODIN & \textbf{70.53 $\pm$ 0.56} & \textbf{42.94\% $\pm$ 0.47\%} & \textbf{0.8679 $\pm$ 0.0016} \\
% & DOCTOR & 71.65 $\pm$ 0.52 & 43.05\% $\pm$ 0.40\% & 0.8635 $\pm$ 0.0016 \\
% & RelU & 86.90 $\pm$ 2.78 & 52.71\% $\pm$ 2.41\% & 0.8185 $\pm$ 0.0065 \\
% \cdashline{2-5}
% & \RobustRad \rule{0pt}{2.2ex} & 76.91 $\pm$ 1.52 & 46.43\% $\pm$ 1.65\% & 0.8502 $\pm$ 0.0031 \\
% & \RobustRadFast  & 76.72 $\pm$ 0.61 & 45.36\% $\pm$ 0.59\% & 0.8524 $\pm$ 0.0017 \\
% & \RobustRadBB  & 72.28 $\pm$ 0.51 & 43.00\% $\pm$ 0.16\% & 0.8592 $\pm$ 0.0016 \\
% \hline
\multirow{9}{*}{ResNet110} & \multicolumn{4}{l}{\textbf{Baseline}\rule{0pt}{2ex}}           \\ \cdashline{2-5}
& MSR & 44.14 $\pm$ 0.59 & 44.09\% $\pm$ 0.77\% & 0.8723 $\pm$ 0.0025 \\
& ODIN & \add{42.09} $\pm$ \add{0.99} & \add{41.84\%} $\pm$ \add{0.36\%} & \add{0.8818} $\pm$ \add{0.0012} \\
& DOCTOR & \add{43.43} $\pm$ \add{1.13} & \add{44.45\%} $\pm$ \add{1.50\%} & \add{0.8798} $\pm$ \add{0.0016} \\
& RelU & 60.71 $\pm$ 11.72 & 68.60\% $\pm$ 9.70\% & 0.8225 $\pm$ 0.0376 \\
\cdashline{2-5}
& \multicolumn{4}{l}{\textbf{Our methods}\rule{0pt}{2ex}}                                            \\ \cdashline{2-5}
& \RobustRad \rule{0pt}{2.2ex} & 39.43 $\pm$ 0.42 & 38.94\% $\pm$ 0.79\% & 0.8844 $\pm$ 0.0010 \\
& \RobustRadFast  & \textbf{39.36 $\pm$ 0.55} & \textbf{38.16\% $\pm$ 1.01\%} & \textbf{0.8874 $\pm$ 0.0014} \\
& \RobustRadBB  & 40.36 $\pm$ 0.27 & 39.00\% $\pm$ 0.22\% & 0.8857 $\pm$ 0.0013 \\
\hline
\end{tabular}
}
\caption{Main results for our methods and baselines. We test our methods on two datasets: CIFAR10 and CIFAR100, with two architectures: WideResNet(WRN)\cite{zagoruyko2016wrn} and DenseNet\cite{huang2017densely}. For each method, we display three metrics: AURC, FPR95 and AUROC. For AURC and FPR95, lower is better. For AUROC, higher is better. Our methods consistently outperform the baselines over these benchmarks. }
\label{tab:MainResults}
\end{table*}

==> tables/omix_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!h]
\centering
\begin{tabular}{c|l|c|c|c}
\hline
\multicolumn{5}{c}{CIFAR10}                                            \\ \hline
 & Method               & AURC  $\times$ 1000 $\downarrow$& FPR@95\%TPR $\downarrow$& AUROC $\uparrow$  \\
\hline
\multirow{9}{*}{WRN-28}& \multicolumn{4}{l}{\textbf{Baseline}\rule{0pt}{2ex}}                                           \\ \cdashline{2-5}
& MSR & 2.14 $\pm$ 0.15 & 11.84\% $\pm$ 1.71\% & 0.9535 $\pm$ 0.0020 \\
& ODIN & 2.12 $\pm$ 0.23 & 12.03\% $\pm$ 1.74\% & 0.9551 $\pm$ 0.0041 \\
& DOCTOR & 2.25 $\pm$ 0.30 & 12.63\% $\pm$ 1.48\% & 0.9541 $\pm$ 0.0058 \\
& RelU & 2.73 $\pm$ 0.79 & 27.26\% $\pm$ 12.54\% & 0.9407 $\pm$ 0.0157 \\
\cdashline{2-5}
& \multicolumn{4}{l}{\textbf{Our methods}\rule{0pt}{2ex}}                                            \\ \cdashline{2-5}
& RR(Ours)\rule{0pt}{2.2ex} & 1.97 $\pm$ 0.23 & \textbf{11.69\% $\pm$ 0.86\%} & 0.9622 $\pm$ 0.0024 \\
& RR-fast(Ours) & \textbf{1.62 $\pm$ 0.06} & 12.89\% $\pm$ 0.71\% & \textbf{0.9638 $\pm$ 0.0020} \\
& RR-Blackbox(Ours) & 1.92 $\pm$ 0.07 & 11.82\% $\pm$ 1.55\% & 0.9579 $\pm$ 0.0017 \\
\hline
\multicolumn{5}{c}{CIFAR100}\\ \hline
\multirow{9}{*}{WRN-28} & \multicolumn{4}{l}{\textbf{Baseline}\rule{0pt}{2ex}}                                           \\ \cdashline{2-5}
& MSR & 35.35 $\pm$ 0.36 & 36.06\% $\pm$ 0.65\% & 0.9008 $\pm$ 0.0009 \\
& ODIN & 35.37 $\pm$ 0.36 & 36.13\% $\pm$ 0.59\% & \textbf{0.9009 $\pm$ 0.0009} \\
& DOCTOR & 35.72 $\pm$ 0.34 & 36.86\% $\pm$ 0.54\% & 0.8999 $\pm$ 0.0016 \\
& RelU & 39.52 $\pm$ 1.78 & 40.91\% $\pm$ 4.12\% & 0.8806 $\pm$ 0.0055 \\
\cdashline{2-5}
& \multicolumn{4}{l}{\textbf{Our methods}\rule{0pt}{2ex}}                                            \\ \cdashline{2-5}
& RR(Ours)\rule{0pt}{2.2ex} & 36.69 $\pm$ 0.31 & 37.85\% $\pm$ 0.53\% & 0.8921 $\pm$ 0.0010 \\
& RR-fast(Ours) & 36.58 $\pm$ 0.40 & 38.96\% $\pm$ 0.83\% & 0.8929 $\pm$ 0.0013 \\
& RR-Blackbox(Ours) &\textbf{35.14 $\pm$ 0.53} & \textbf{35.31\% $\pm$ 1.07\%} & 0.8981 $\pm$ 0.0021 \\
\hline
\end{tabular}
\caption{Openmix results for our methods and baselines.  We test our methods on two datasets: CIFAR10 and CIFAR100, with two architectures: WideResNet(WRN)\cite{zagoruyko2016wrn} and DenseNet\cite{huang2017densely}. For each method, we display three metrics: AURC, FPR95 and AUROC. For AURC and FPR95, lower is better. For AUROC, higher is better. Our methods are best among all methods except for AUROC metric on CIFAR100.}
\label{tab:OmixResults}
\end{table}

==> tables/wb_evaluation.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{lllllll}
    \hline
    Method & AUROC\_mean $\uparrow$ & AUROC\_std & FPR@95\_mean $\downarrow$ & FPR@95\_std & AURC\_mean $\downarrow$ & AURC\_std \\ 
    \hline
    \multicolumn{7}{c}{CIFAR10}\\
    \hline
        HPS & 0.8846 & 0.018 & 30.53\% & 4.87\% & 5.44 & 0.68  \\ 
        MSR & 0.9017 & 0.0074 & 35.77\% & 11.09\% & 4.31 & 0.45  \\ 
        tfDOCTOR & 0.8617 & 0.0354 & 30.09\% & 7.95\% & 7.24 & 1.56  \\ 
        logiDiff & 0.9081 & 0.003 & 29.73\% & 6.57\% & 3.82 & 0.22  \\ \hline
        thr & 0.9069 & 0.0066 & 31.48\% & 9.86\% & 3.96 & 0.37  \\ 
        DOCTOR & 0.8596 & 0.0369 & 32.03\% & 7.82\% & 6.96 & 1.74  \\ 
        ODIN & 0.9085 & 0.0055 & 32.45\% & 9.83\% & 3.93 & 0.6 \\ 
    \hline
    \multicolumn{7}{c}{CIFAR100}\\
    \hline
        HPS & 0.8534 & 0.0014 & 72.78\% & 1.49\% & 50.23 & 0.66  \\ 
        MSR & 0.8679 & 0.0023 & 57.87\% & 1.16\% & 51.01 & 0.56  \\ 
        tfDOCTOR & 0.8485 & 0.0014 & 57.16\% & 0.62\% & 60.46 & 0.55  \\ 
        logiDiff & 0.8702 & 0.0015 & 61.46\% & 2.33\% & 46.11 & 0.43 \\ \hline
        thr & 0.8755 & 0.0018 & 59.24\% & 1.21\% & 45.04 & 0.45  \\ 
        DOCTOR & 0.8669 & 0.0013 & 59.25\% & 0.47\% & 49.82 & 0.36  \\ 
        ODIN & 0.873 & 0.0022 & 61.64\% & 2.12\% & 46.35 & 0.47  \\ 
    \hline
    \multicolumn{7}{c}{ImageNet}\\    
    \hline
        HPS & 0.8289 & 0.0036 & 77.84\% & 1.26\% & 58.75 & 0.53  \\ 
        MSR & 0.8066 & 0.0003 & 67.63\% & 0.24\% & 73.87 & 0.2  \\ 
        tfDOCTOR & 0.7802 & 0.0004 & 70.82\% & 0.09\% & 82.48 & 0.23  \\ 
        logiDiff & 0.8593 & 0.0002 & 70.66\% & 0.02\% & 51.61 & 0.14 \\ \hline
        thr & 0.8583 & 0.0002 & 66.79\% & 0.05\% & 52.1 & 0.13  \\ 
        DOCTOR & 0.861 & 0.0044 & 65.43\% & 1.67\% & 53.52 & 1.97  \\ 
        ODIN & 0.8629 & 0.0024 & 66.22\% & 1.51\% & 52.4 & 0.96  \\ 
    \hline
    \end{tabular}
    \caption{White box evaluation results. Experiments are conducted over 10 random validation-test splits.}
\end{table*}
